Content Sequencing and its Impact on Student Learning in Electromagnetism: Theory and Experiment

We investigate the impact of content sequencing on student learning outcomes in a first-year university electromagnetism course. Using a custom-built online system, the McGill Learning Platform (McLEAP), we test student problem-solving performance as a function of the sequence in which the students are presented aspects of new material. New material was divided into the three categories of conceptual, theoretical and example-based content. Here, we present findings from a two-year study with over 1000 students participating. We find that content sequencing has a significant impact on learning outcomes in our study: students presented with conceptual content first perform significantly better on our assessment than those presented with theoretical content. To explain these results, we propose the Content Cube as an extension to the the mental model frameworks. Additionally, we find that instructors' preferences for content sequencing differ significantly from that of students. We discuss how this information can be used to improve course instruction and student learning, and motivate future work building upon our presented results to study the impact of additional factors on student performance.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
